Smooth limits of plane curves of prime degree and Markov numbers

For prime degree hypersurfaces of dimension at least 3, Mori asked if every smooth proper limit is still a hypersurface. Interestingly in dimensions 1 and 2, this is not the case. For example, Griffin constructed explicit families of quintic curves that give counterexamples in dimension 1 (Horikawa constructed similar examples for quintics in dimension 2). In this paper we propose a conjecture explaining these examples using Hacking and Prokhorov's work on Q-Gorenstein limits of the projective plane. In particular, if p is a prime number that is not a Markov number, we conjecture that any smooth projective limit of plane curves of degree p is a plane curve. The main results are to prove this conjecture for degree 7 curves and to extend Griffin's counterexamples to all prime numbers that are also Markov numbers.

==> Pics/M1G2.tex <==
\begin{tikzpicture}[gren0/.style = {draw, circle,fill=greener!80,scale=.7},gren/.style ={draw, circle, fill=greener!80,scale=.4}]
\node[gren] at (-.6,0) (1){$2$};
\node[scale=.5] (1) at (0,0) (2){};
\node[gren0] at (.6,0) (3){};
\draw (1)--(2);
\draw (2)--(3);
\filldraw [orange!60,scale=.11] (0,0) circle () {};
\end{tikzpicture}

==> Pics/M2G2a.tex <==
\begin{tikzpicture}[gren0/.style = {draw, circle,fill=greener!80,scale=.7},gren/.style ={draw, circle, fill=greener!80,scale=.4}] 
\node[scale=.5] at (0,0) (1){};
\node[gren] at (.6,-.2) (3){$2$};
\node[gren] at (.6,.2) (4){$2$};
\draw (1)--(3);
\draw (1)--(4);
\filldraw [orange!60,scale=.11] (0,0) circle () {};
\end{tikzpicture} 
